Assessing the alignment accuracy of state-of-the-art deterministic fabrication methods for single quantum dot devices

The realization of efficient quantum light sources relies on the integration of self-assembled quantum dots (QDs) into photonic nanostructures with high spatial positioning accuracy. In this work, we present a comprehensive investigation of the QD position accuracy, obtained using two marker-based QD positioning techniques, photoluminescence (PL) and cathodoluminescence (CL) imaging, as well as using a marker-free in-situ electron beam lithography (in-situ EBL) technique. We employ four PL imaging configurations with three different image processing approaches and compare them with CL imaging. We fabricate circular mesa structures based on the obtained QD coordinates from both PL and CL image processing to evaluate the final positioning accuracy. This yields final position offset of the QD relative to the mesa center of $\mu_x$ = (-40$\pm$58) nm and $\mu_y$ = (-39$\pm$85) nm with PL imaging and $\mu_x$ = (-39$\pm$30) nm and $\mu_y$ = (25$\pm$77) nm with CL imaging, which are comparable to the offset $\mu_x$ = (20$\pm$40) nm and $\mu_y$ = (-14$\pm$39) nm obtained using the in-situ EBL method. We discuss the possible causes of the observed offsets, which are significantly larger than the QD localization uncertainty obtained from simply imaging the QD light emission from an unstructured wafer. Our study highlights the influences of the image processing technique and the subsequent fabrication process on the final positioning accuracy for a QD placed inside a photonic nanostructure.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> settings.tex <==
\usepackage[intlimits]{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{braket}
\usepackage{color}
\usepackage{float}
%\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{glossaries}
\usepackage[normalem]{ulem}
%\usepackage[colorlinks=true,
%            linkcolor=NavyBlue,
%            citecolor=NavyBlue,
%            filecolor=NavyBlue,
%            urlcolor=NavyBlue
%           ]{hyperref}
            
\usepackage[colorlinks=true,
            linkcolor=black,
            citecolor=black,
            filecolor=black,
            urlcolor=black
            ]{hyperref}
\usepackage[utf8]{inputenc}
\usepackage[version=4]{mhchem}
\usepackage{multirow}
\usepackage{soul}
\usepackage{tabularx}
\usepackage{units}
\usepackage[dvipsnames]{xcolor}

\usepackage{dcolumn}
\usepackage{float}
%\usepackage{siunitx}
%\usepackage{mathptmx}
\usepackage{booktabs}

\newcommand{\rev}{\textcolor{red}}
%\bibliographystyle{chem-acs}


\setacronymstyle{long-short}
\newacronym{qd}{QD}{quantum dot}
\newacronym{pl}{PL}{Photoluminescence}
\newacronym{cl}{CL}{Cathodoluminescence}
\newacronym{gaas}{GaAs}{Gallium Arsenide}
\newacronym{ingaas}{InGaAs}{Indium Gallium Arsenide}
\newacronym{ebl}{EBL}{Electron beam lithography}

\newacronym{vis}{VIS}{visible}
\newacronym{nir}{NIR}{near-infrared}
\newacronym{uv}{UV}{ultraviolet}
\newacronym{mse}{MSE}{mean squared error}
\newacronym{si}{SI}{Supporting Information}

% autoref prefixes
\def\sectionautorefname{Sect.}
\def\figureautorefname{Fig.}
\def\tableautorefname{Table}
\def\equationautorefname{Eq.}
\def\noteautorefname{Supplementary Note}

\newcommand{\corr}{\textcolor{red}}
\renewcommand{\thetable}{\arabic{table}}

\newlabel{fig:mm-PL}{{S1}{2}{figure caption text1. \relax }{figure.caption.1}{}}







